On the Enumeration of Circulant Graphs of Prime-Power Order: the case of $p^3$

A well-known problem in Algebraic Combinatorics, is the enumeration of circulant graphs. The failure of Adam's Conjecture for such graphs with order containing a repeated prime, led researchers to investigate the problem using two different methods, namely the multiplier method and the structural method. The former makes use of isomorphism theorems whereas the latter involves Schur rings. Both these methods have already been used to count the number of non-isomorphic circulants of order $p^2$. This research focuses on the extension of these two methods to enumerate circulants of order $p^3$, in particular for $p=3$ and $p=5$, through the use of the computer package GAP.

==> generating_functions.tex <==
\section{Generating Functions for Circulants of order 27, Undirected}

\begin{align*}
A_{1}[u;27](t)=t^{26}+t^{24}+t^{20}+t^{18}+t^8+t^6+t^2+1\\
\end{align*}

\begin{align*}
A_{21}[u;27](t)=t^{26}+3t^{24}+10t^{22}+34t^{20}+83t^{18}+147t^{16}\\
+194t^{14}+194t^{12}+147t^{10}+83t^8+34t^6+10t^4+3t^2+1
\end{align*}

\begin{align*}
A_{22}[u;27](t)=t^{26}+2t^{24}+2t^{22}+3t^{20}+5t^{18}+6t^{16}+5t^{14}+5t^{12}+\\
6t^{10}+5t^8+3t^6+2t^4+2t^2+1
\end{align*}

\begin{align*}
A_{2}[u;27](t)=t^{24}+8t^{22}+31t^{20}+78t^{18}+141t^{16}+189t^{14}+189t^{12}+\\
141t^{10}+78t^8+31t^6+8t^4+t^2
\end{align*}

\begin{align*}
A_{31}[u;27](t)=t^{26}+t^{24}+2t^{20}+2t^{18}+2t^{14}+2t^{12}+2t^8+2t^6+t^2+1
\end{align*}

\begin{align*}
A_{32}[u;27](t)=t^{26}+t^{24}+t^{20}+t^{18}+t^8+t^6+t^2+1
\end{align*}

\begin{align*}
A_{3}[u;27](t)=t^{20}+t^{18}+2t^{14}+2t^{12}+t^8+t^6
\end{align*}

\begin{align*}
A_{41}[u;27](t)=t^{26}+2t^{24}+2t^{22}+2t^{20}+t^{18}+t^8+2t^6+2t^4+2t^2+1
\end{align*}

\begin{align*}
A_{42}[u;27](t)=t^{26}+t^{24}+t^{20}+t^{18}+t^8+t^6+t^2+1
\end{align*}

\begin{align*}
A_{4}[u;27](t)&=t^{24}+2t^{22}+t^{20}+t^6+2t^4+t^2\\
\end{align*}

\begin{align*}
A_{51}[u;27](t)&=t^{26}+2t^{24}+2t^{22}+3t^{20}+3t^{18}+2t^{16}+3t^{14}+3t^{12}+\\
&2t^{10}+3t^8+3t^6+2t^4+2t^2+1
\end{align*}

\begin{align*}
A5_{21}[u;27](t)&=t^{26}+2t^{24}+2t^{22}+2t^{20}+t^{18}+t^8+2t^6+2t^4+2t^2+1\\
\end{align*}

\begin{align*}
A5_{22}[u;27](t)&=t^{26}+t^{24}+2t^{20}+2t^{18}+2t^{14}+2t^{12}+2t^8+2t^6+t^2+1
\end{align*}

\begin{align*}
A5_{23}[u;27](t)=t^{26}+t^{24}+t^{20}+t^{18}+t^8+t^6+t^2+1
\end{align*}

\begin{align*}
A_{52}[u;27](t)=t^{26}+2t^{24}+2t^{22}+3t^{20}+2t^{18}+2t^{14}+2t^{12}+2t^8+3t^6+2t^4+2t^2+1
\end{align*}

\begin{align*}
A_{5}[u;27](t)=t^{18}+2t^{16}+t^{14}+t^{12}+2t^{10}+t^8
\end{align*}

%\begin{multline*}
\begin{align*}
Total[u;27](t)&=A_{1}+A_{2}+A_{3}+A_{4}+A_{5}\\
&=t^{26}+3t^{24}+10t^{22}+34t^{20}+81t^{18}+143t^{16}+192t^{14}+\\
&192t^{12}+143t^{10}+81t^8+34t^6+10t^4+3t^2+1\\
\end{align*}
%\end{multline*}

\newpage
\section{Generating Functions for Circulants of Order 27, Directed}
\begin{align*}
A_{1}[d;27](t)&=t^{26}+t^{25}+t^{24}+t^{23}+t^{22}+t^{21}+t^{20}+t^{19}+t^{18}+t^{17}+\\
&t^{16}+t^{15}+t^{14}+t^{13}+t^{12}+t^{11}+t^{10}+t^9+t^8+t^7+t^6+t^5+t^4+t^3+t^2+t+1\\
\end{align*}

\begin{align*}
A_{21}[d;27](t)&=t^{26}+3t^{25}+23t^{24}+152t^{23}+850t^{22}+\\
&3680t^{21}+12850t^{20}+36606t^{19}+86919t^{18}+173701t^{17}+\\
&295311t^{16}+429388t^{15}+536810t^{14}+577996t^{13}+536810t^{12}+\\
&429388t^{11}+295311t^{10}+173701t^9+86919t^8+36606t^7+12850t^6+\\
&3680t^5+850t^4+152t^3+23t^2+3t+1\\
\end{align*}

\begin{align*}
A_{22}[d;27](t)&=t^{26}+2t^{25}+6t^{24}+11t^{23}+22t^{22}+38t^{21}+\\
&65t^{20}+92t^{19}+129t^{18}+172t^{17}+214t^{16}+235t^{15}+263t^{14}+\\
&276t^{13}+263t^{12}+235t^{11}+214t^{10}+172t^9+129t^8+92t^7+\\
&65t^6+38t^5+22t^4+11t^3+6t^2+2t+1\\
\end{align*}

\begin{align*}
A_{2}[d;27](t)&=t^{25}+17t^{24}+141t^{23}+828t^{22}+3642t^{21}+\\
&12785t^{20}+36514t^{19}+86790t^{18}+173529t^{17}+295097t^{16}+\\
&429153t^{15}+536547t^{14}+577720t^{13}+536547t^{12}+429153t^{11}+\\
&295097t^{10}+173529t^9+86790t^8+36514t^7+12785t^6+3642t^5+828t^4+\\
&141t^3+17t^2+t\\
\end{align*}

\begin{align*}
A_{31}[d;27](t)&=t^{26}+t^{25}+t^{24}+2t^{23}+2t^{22}+2t^{21}+6t^{20}+\\
&6t^{19}+6t^{18}+10t^{17}+10t^{16}+10t^{15}+14t^{14}+14t^{13}+14t^{12}+\\
&10t^{11}+10t^{10}+10t^9+6t^8+6t^7+6t^6+2t^5+2t^4+2t^3+t^2+t+1\\
\end{align*}

\begin{align*}
A_{32}[d;27](t)&=t^{26}+t^{25}+t^{24}+t^{23}+t^{22}+t^{21}+t^{20}+t^{19}+\\
&t^{18}+t^{17}+t^{16}+t^{15}+2t^{14}+2t^{13}+2t^{12}+t^{11}+t^{10}+\\
&t^9+t^8+t^7+t^6+t^5+t^4+t^3+t^2+t+1\\
\end{align*}

\begin{flalign*}
A_{3}[d;27](t)&=t^{23}+t^{22}+t^{21}+5t^{20}+5t^{19}+5t^{18}+9t^{17}+\\
&9t^{16}+9t^{15}+12t^{14}+12t^{13}+12t^{12}+9t^{11}+9t^{10}+9t^9+\\
&5t^8+5t^7+5t^6+t^5+t^4+t^3\\
\end{flalign*}

\begin{align*}
A_{41}[d;27](t)&=t^{26}+2t^{25}+6t^{24}+10t^{23}+14t^{22}+10t^{21}+\\
&6t^{20}+2t^{19}+t^{18}+t^{17}+2t^{16}+6t^{15}+10t^{14}+14t^{13}+\\
&10t^{12}+6t^{11}+2t^{10}+t^9+t^8+2t^7+6t^6+10t^5+14t^4+10t^3+6t^2+2t+1\\
\end{align*}

\begin{align*}
A_{42}[d;27](t)&=t^{26}+t^{25}+t^{24}+t^{23}+2t^{22}+t^{21}+t^{20}+t^{19}+\\
&t^{18}+t^{17}+t^{16}+t^{15}+t^{14}+2t^{13}+\\
&t^{12}+t^{11}+t^{10}+t^9+t^8+t^7+t^6+t^5+2t^4+t^3+t^2+t+1\\
\end{align*}

\begin{align*}
A_{4}[d;27](t)&=t^{25}+5t^{24}+9t^{23}+12t^{22}+9t^{21}+5t^{20}+t^{19}+\\
&t^{16}+5t^{15}+9t^{14}+12t^{13}+9t^{12}+\\
&5t^{11}+t^{10}+t^7+5t^6+9t^5+12t^4+9t^3+5t^2+t\\
\end{align*}

\begin{align*}
A_{51}[d;27](t)&=t^{26}+2t^{25}+6t^{24}+11t^{23}+18t^{22}+20t^{21}+\\
&29t^{20}+38t^{19}+47t^{18}+64t^{17}+86t^{16}+\\
&91t^{15}+109t^{14}+124t^{13}+109t^{12}+91t^{11}+86t^{10}+64t^9+\\
&47t^8+38t^7+29t^6+20t^5+18t^4+11t^3+6t^2+2t+1\\
\end{align*}

\begin{align*}
A5_{21}[d;27](t)&=t^{26}+2t^{25}+6t^{24}+10t^{23}+14t^{22}+10t^{21}+\\
&6t^{20}+2t^{19}+t^{18}+t^{17}+4t^{16}+10t^{15}+\\
&20t^{14}+26t^{13}+20t^{12}+10t^{11}+4t^{10}+t^9+t^8+2t^7+6t^6+\\
&10t^5+14t^4+10t^3+6t^2+2t+1\\
\end{align*}
\begin{align*}
A5_{22}[d;27](t)&=t^{26}+t^{25}+t^{24}+2t^{23}+4t^{22}+2t^{21}+6t^{20}+\\
&10t^{19}+6t^{18}+10t^{17}+20t^{16}+10t^{15}+\\
&14t^{14}+26t^{13}+14t^{12}+10t^{11}+20t^{10}+10t^9+6t^8+10t^7+\\
&6t^6+2t^5+4t^4+2t^3+t^2+t+1\\
\end{align*}

\begin{align*}
A5_{23}[d;27](t)&=t^{26}+t^{25}+t^{24}+t^{23}+2t^{22}+t^{21}+t^{20}+t^{19}+t^{18}+t^{17}+2t^{16}+t^{15}+\\
&2t^{14}+4t^{13}+2t^{12}+t^{11}+2t^{10}+t^9+t^8+t^7+t^6+t^5+2+t^4+t^3+t^2+t+1\\
\end{align*}

\begin{align*}
A_{52}[d;27](t)&=t^{26}+2t^{25}+6t^{24}+11t^{23}+16t^{22}+11t^{21}+11t^{20}+11t^{19}+\\
&6t^{18}+10t^{17}+22t^{16}+19t^{15}+32t^{14}+48t^{13}+32t^{12}+19t^{11}+22t^{10}+\\
&10t^9+6t^8+11t^7+11t^6+11t^5+16t^4+11t^3+6t^2+2t+1\\
\end{align*}

\begin{align*}
A_{5}[d;27](t)&=2t^{22}+9t^{21}+18t^{20}+27t^{19}+41t^{18}+54t^{17}+64t^{16}+72t^{15}+77t^{14}+76t^{13}+\\
&77t^{12}+72t^{11}+64t^{10}+54t^9+41t^8+27t^7+ 18t^6+9t^5+2t^4\\
\end{align*}


\begin{align*}
Total[d;27](t)&=A_{1}+A_{2}+A_{3}+A_{4}+A_{5}\\
&=t^{26}+3t^{25}+23t^{24}+152t^{23}+844t^{22}+3662t^{21}+12814t^{20}+36548t^{19}+\\
&86837t^{18}+173593t^{17}+295172t^{16}+429240t^{15}+536646t^{14}+577821t^{13}+\\
&536646t^{12}+429240t^{11}+295172t^{10}+173593t^9+86837t^8+36548t^7+12814t^6+\\
&3662t^5+844t^4+152t^3+23t^2+3t+1\\
\end{align*}

\newpage
\section{Generating Functions for Circulants of Order 125, Undirected}
\begin{align*}
A_{1}[u;125](t)&=t^{124}+t^{122}+t^{120}+t^{114}+t^{112}+t^{110}+t^{104}+t^{102}+\\
&t^{100}+t^{74}+t^{72}+t^{70}+t^{64}+t^{62}+t^{60}+t^{54}+t^{52}+t^{50}+\\
&t^{24}+t^{22}+t^{20}+t^{14}+t^{12}+t^{10}+t^4+t^2+1
\end{align*}

\begin{align*}
A_{21}[u;125](t)&=t^{124}+3t^{122}+45t^{120}+774t^{118}+\\
&11207t^{116}+129485t^{114}+1229667t^{112}+9836040t^{110}+\\
&67622817t^{108}+405732239t^{106}+2150382717t^{104}+10165427246t^{102}+\\
&43203078063t^{100}+166165626045t^{98}+581579741555t^{96}+\\
&1861055001312t^{94}+ 5466849219029t^{92}+14792650395167t^{90}+\\
&36981626386305t^{88}+85641660167910t^{86}+184129570243991t^{84}+\\
&368259138707289t^{82}+686301123821491t^{80}+\\
&1193567168911620t^{78}+1939546652300505t^{76}+2948110907204795t^{74}+\\
&4195388602835609t^{72}+5593851464940846t^{70}+6992314336474163t^{68}+\\
&8197885767577933t^{66}+9017674350348587t^{64}+9308567065124256t^{62}+\\
&9017674350348587t^{60}+8197885767577933t^{58}+6992314336474163t^{56}+\\
&5593851464940846t^{54}+4195388602835609t^{52}+2948110907204795t^{50}+\\
&1939546652300505t^{48}+1193567168911620t^{46}+686301123821491t^{44}+\\
&368259138707289t^{42}+184129570243991t^{40}+85641660167910t^{38}+\\
&36981626386305t^{36}+14792650395167t^{34}+ 5466849219029t^{32}+1861055001312t^{30}+\\
&581579741555t^{28}+166165626045t^{26}+43203078063t^{24}+10165427246t^{22}+\\
&2150382717t^{20}+405732239t^{18}+67622817t^{16}+9836040t^{14}+1229667t^{12}+\\
&129485t^{10}+11207t^8+774t^6+45t^4+3t^2+1\\
\end{align*}


\begin{align*}
A_{22}[u;125](t)&=t^{124}+2t^{122}+8t^{120}+22t^{118}+51t^{116}+\\
&81t^{114}+108t^{112}+146t^{110}+271t^{108}+517t^{106}+805t^{104}+\\
&980t^{102}+1093t^{100}+1485t^{98}+2455t^{96}+3642t^{94}+4324t^{92}+\\
&4357t^{90}+4875t^{88}+6930t^{86}+9826t^{84}+11394t^{82}+10901t^{80}+\\
&10560t^{78}+13050t^{76}+17450t^{74}+19872t^{72}+18308t^{70}+15954t^{68}+\\
&17094t^{66}+21374t^{64}+23792t^{62}+21374t^{60}+17094t^{58}+15954t^{56}+\\
&18308t^{54}+19872t^{52}+17450t^{50}+13050t^{48}+10560t^{46}+10901t^{44}+\\
&11394t^{42}+9826t^{40}+6930t^{38}+4875t^{36}+4357t^{34}+4324t^{32}+3642t^{30}+\\
&2455t^{28}+1485t^{26}+1093t^{24}+980t^{22}+805t^{20}+517t^{18}+271t^{16}+\\
&146t^{14}+108t^{12}+81t^{10}+51t^8+ 22t^6+8t^4+2t^2+1\\
\end{align*}

\begin{align*}
A_{2}[u;&125](t)=t^{122}+37t^{120}+752t^{118}+11156t^{116}+129404t^{114}+\\
&1229559t^{112}+9835894t^{110}+67622546t^{108}+405731722t^{106}+\\
&2150381912t^{104}+10165426266t^{102}+43203076970t^{100}+166165624560t^{98}+\\
&581579739100t^{96}+1861054997670t^{94}+5466849214705t^{92}+14792650390810t^{90}+\\
&36981626381430t^{88}+85641660160980t^{86}+184129570234165t^{84}+ 368259138695895t^{82}+\\
&686301123810590t^{80}+1193567168901060t^{78}+1939546652287455t^{76}+\\
&2948110907187345t^{74}+4195388602815737t^{72}+5593851464922538t^{70}+\\
&6992314336458209t^{68}+8197885767560839t^{66}+9017674350327213t^{64}+\\
&9308567065100464t^{62}+9017674350327213t^{60}+8197885767560839t^{58}+\\
&6992314336458209t^{56}+5593851464922538t^{54}+ 4195388602815737t^{52}+\\
&2948110907187345t^{50}+1939546652287455t^{48}+1193567168901060t^{46}+\\
&686301123810590t^{44}+368259138695895t^{42}+184129570234165t^{40}+85641660160980t^{38}+\\
&36981626381430t^{36}+14792650390810t^{34}+ 5466849214705t^{32}+1861054997670t^{30}+\\
&581579739100t^{28}+166165624560t^{26}+43203076970t^{24}+10165426266t^{22}+\\
&2150381912t^{20}+405731722t^{18}+67622546t^{16}+9835894t^{14}+1229559t^{12}+\\
&129404t^{10}+11156t^8+752t^6+37t^4+t^2
\end{align*}

\begin{align*}
A_{31}[u;125](t)&=t^{124}+t^{122}+t^{120}+2t^{114}+2t^{112}+2t^{110}+8t^{104}+8t^{102}+\\
&8t^{100}+22t^{94}+22t^{92}+22t^{90}+51t^{84}+51t^{82}+51t^{80}+80t^{74}+80t^{72}+\\
&80t^{70}+96t^{64}+96t^{62}+96t^{60}+80t^{54}+80t^{52}+80t^{50}+51t^{44}+51t^{42}+\\
&51t^{40}+22t^{34}+22t^{32}+22t^{30}+8t^{24}+8t^{22}+8t^{20}+2t^{14}+2t^{12}+2t^{10}+t^4+t^2+1
\end{align*}

\begin{align*}
A_{32}[u;125](t)&=t^{124}+t^{122}+t^{120}+t^{114}+t^{112}+t^{110}+t^{104}+t^{102}+t^{100}+t^{74}+\\
&t^{72}+t^{70}+2t^{64}+2t^{62}+2t^{60}+t^{54}+t^{52}+t^{50}+t^{24}+t^{22}+\\
&t^{20}+t^{14}+t^{12}+t^{10}+t^4+t^2+1
\end{align*}

\begin{align*}
A_{3}[u;125](t)&=t^{114}+t^{112}+t^{110}+7t^{104}+7t^{102}+7t^{100}+22t^{94}+22t^{92}+22t^{90}+\\
&51t^{84}+51t^{82}+51t^{80}+79t^{74}+79t^{72}+79t^{70}+94t^{64}+94t^{62}+94t^{60}+79t^{54}+79t^{52}+\\
&79t^{50}+51t^{44}+51t^{42}+51t^{40}+22t^{34}+22t^{32}+22t^{30}+7t^{24}+7t^{22}+7t^{20}+t^{14}+\\
&t^{12}+t^{10}
\end{align*}

\begin{align*}
A_{41}[u;125](t)&=t^{124}+2t^{122}+8t^{120}+22t^{118}+51t^{116}+80t^{114}+96t^{112}+80t^{110}+\\
&51t^{108}+22t^{106}+8t^{104}+2t^{102}+t^{100}+t^{74}+2t^{72}+8t^{70}+22t^{68}+51t^{66}+80t^{64}+\\
&96t^{62}+80t^{60}+51t^{58}+22t^{56}+8t^{54}+2t^{52}+t^{50}+t^{24}+2t^{22}+8t^{20}+22t^{18}+\\
&51t^{16}+80t^{14}+96t^{12}+80t^{10}+51t^8+22t^6+8t^4+2t^2+1
\end{align*}

\begin{align*}
A_{42}[u;125](t)&=t^{124}+t^{122}+t^{120}+t^{114}+2t^{112}+t^{110}+t^{104}+t^{102}+\\
&t^{100}+t^{74}+t^{72}+t^{70}+t^{64}+2t^{62}+t^{60}+t^{54}+t^{52}+t^{50}+t^{24}+t^{22}+\\
&t^{20}+t^{14}+2t^{12}+t^{10}+t^4+t^2+1
\end{align*}

\begin{align*}
A_{4}[u;125](t)&=t^{122}+7t^{120}+22t^{118}+51t^{116}+79t^{114}+94t^{112}+79t^{110}+\\
&51t^{108}+22t^{106}+7t^{104}+t^{102}+t^{72}+7t^{70}+22t^{68}+51t^{66}+79t^{64}+94t^{62}+\\
&79t^{60}+51t^{58}+22t^{56}+7t^{54}+t^{52}+t^{22}+7t^{20}+22t^{18}+51t^{16}+79t^{14}+\\
&94t^{12}+79t^{10}+51t^8+22t^6+7t^4+t^2
\end{align*}

\begin{align*}
A_{51}[u;&125](t)=t^{124}+2t^{122}+8t^{120}+22t^{118}+51t^{116}+81t^{114}+100t^{112}+94t^{110}+95t^{108}+\\
&121t^{106}+173t^{104}+208t^{102}+225t^{100}+297t^{98}+491t^{96}+746t^{94}+900t^{92}+889t^{90}+975t^{88}+\\
&1386t^{86}+2006t^{84}+2358t^{82}+2221t^{80}+2112t^{78}+2610t^{76}+3554t^{74}+4104t^{72}+3736t^{70}+\\
&3226t^{68}+3498t^{66}+4478t^{64}+5056t^{62}+4478t^{60}+3498t^{58}+3226t^{56}+3736t^{54}+4104t^{52}+\\
&3554t^{50}+2610t^{48}+2112t^{46}+2221t^{44}+2358t^{42}+2006t^{40}+1386t^{38}+975t^{36}+889t^{34}+\\
&900t^{32}+746t^{30}+491t^{28}+297t^{26}+225t^{24}+208t^{22}+173t^{20}+121t^{18}+95t^{16}+94t^{14}+\\
&100t^{12}+81t^{10}+51t^8+22t^6+8t^4+2t^2+1
\end{align*}

\begin{align*}
A5_{21}[u;125](t)&=t^{124}+2t^{122}+8t^{120}+22t^{118}+51t^{116}+80t^{114}+96t^{112}+80t^{110}+\\
&51t^{108}+22t^{106}+8t^{104}+2t^{102}+t^{100}+t^{74}+4t^{72}+14t^{70}+44t^{68}+99t^{66}+160t^{64}+\\
&188t^{62}+160t^{60}+99t^{58}+44t^{56}+14t^{54}+4t^{52}+t^{50}+t^{24}+2t^{22}+8t^{20}+22t^{18}+\\
&51t^{16}+80t^{14}+96t^{12}+80t^{10}+51t^8+22t^6+8t^4+2t^2+1
\end{align*}

\begin{align*}
A5_{22}[u;125](t)&=t^{124}+t^{122}+t^{120}+2t^{114}+4t^{112}+2t^{110}+8t^{104}+14t^{102}+8t^{100}+\\
&22t^{94}+44t^{92}+22t^{90}+51t^{84}+99t^{82}+51t^{80}+80t^{74}+160t^{72}+80t^{70}+96t^{64}+188t^{62}+\\
&96t^{60}+80t^{54}+160t^{52}+80t^{50}+51t^{44}+99t^{42}+51t^{40}+22t^{34}+44t^{32}+22t^{30}+8t^{24}+\\
&14t^{22}+8t^{20}+2t^{14}+4t^{12}+2t^{10}+t^4+t^2+1
\end{align*}

\begin{align*}
A5_{23}[u;125](t)&=t^{124}+t^{122}+t^{120}+t^{114}+2t^{112}+t^{110}+t^{104}+t^{102}+\\
&t^{100}+t^{74}+2t^{72}+t^{70}+2t^{64}+4t^{62}+2t^{60}+t^{54}+2t^{52}+t^{50}+t^{24}+t^{22}+\\
&t^{20}+t^{14}+2t^{12}+t^{10}+t^4+t^2+1\\
\end{align*}

\begin{align*}
A_{52}[u;&125](t)=t^{124}+2t^{122}+8t^{120}+22t^{118}+51t^{116}+81t^{114}+98t^{112}+\\
&81t^{110}+51t^{108}+22t^{106}+15t^{104}+15t^{102}+8t^{100}+22t^{94}+44t^{92}+22t^{90}+\\
&51t^{84}+99t^{82}+51t^{80}+80t^{74}+162t^{72}+93t^{70}+44t^{68}+99t^{66}+254t^{64}+\\
&372t^{62}+254t^{60}+99t^{58}+44t^{56}+93t^{54}+162t^{52}+80t^{50}+51t^{44}+99t^{42}+\\
&51t^{40}+22t^{34}+44t^{32}+22t^{30}+8t^{24}+15t^{22}+15t^{20}+22t^{18}+51t^{16}+\\
&81t^{14}+98t^{12}+81t^{10}+51t^8+22t^6+8t^4+2t^2+1
\end{align*}

\begin{align*}
A_{5}[u;&125](t)=2t^{112}+13t^{110}+44t^{108}+99t^{106}+158t^{104}+193t^{102}+217t^{100}+\\
&297t^{98}+491t^{96}+724t^{94}+856t^{92}+867t^{90}+975t^{88}+1386t^{86}+1955t^{84}+2259t^{82}+\\
&2170t^{80}+2112t^{78}+2610t^{76}+3474t^{74}+3942t^{72}+3643t^{70}+3182t^{68}+3399t^{66}+4224t^{64}+\\
&4684t^{62}+4224t^{60}+3399t^{58}+3182t^{56}+3643t^{54}+3942t^{52}+3474t^{50}+2610t^{48}+2112t^{46}+\\
&2170t^{44}+2259t^{42}+1955t^{40}+1386t^{38}+975t^{36}+867t^{34}+856t^{32}+724t^{30}+491t^{28}+\\
&297t^{26}+217t^{24}+193t^{22}+158t^{20}+99t^{18}+44t^{16}+13t^{14}+2t^{12}
\end{align*}

\begin{align*}
Total[u;125](t)&=A_{1}+A_{2}+A_{3}+A_{4}+A_{5}\\
&t^{124}+3t^{122}+45t^{120}+774t^{118}+11207t^{116}+129485t^{114}+\\
&1229657t^{112}+9835988t^{110}+67622641t^{108}+ 405731843t^{106}+\\
&2150382085t^{104}+10165426468t^{102}+43203077195t^{100}+\\
&166165624857t^{98}+581579739591t^{96}+1861054998416t^{94}+\\
&5466849215583t^{92}+14792650391699t^{90}+36981626382405t^{88}+\\
&85641660162366t^{86}+184129570236171t^{84}+368259138698205t^{82}+\\
&686301123812811t^{80}+1193567168903172t^{78}+1939546652290065t^{76}+\\
&2948110907190899t^{74}+4195388602819760t^{72}+5593851464926268t^{70}+\\
&6992314336461413t^{68}+8197885767564289t^{66}+\\
&9017674350331611t^{64}+9308567065105337t^{62}+9017674350331611t^{60}+\\
&8197885767564289t^{58}+6992314336461413t^{56}+5593851464926268t^{54}+\\
&4195388602819760t^{52}+2948110907190899t^{50}+1939546652290065t^{48}+\\
&1193567168903172t^{46}+686301123812811t^{44}+368259138698205t^{42}+\\
&184129570236171t^{40}+85641660162366t^{38}+36981626382405t^{36}+\\
&14792650391699t^{34}+5466849215583t^{32}+1861054998416t^{30}+\\
&581579739591t^{28}+166165624857t^{26}+43203077195t^{24}+\\
&10165426468t^{22}+2150382085t^{20}+405731843t^{18}+67622641t^{16}+\\
&9835988t^{14}+1229657t^{12}+129485t^{10}+11207t^8+\\
&774t^6+45t^4+3t^2+1
\end{align*}

\newpage
\section{Generating Functions for Circulants of Order 125, Directed}
\begin{align*}
A_{1}[d;&125](t)=t^{124}+t^{123}+2t^{122}+t^{121}+t^{120}+t^{119}+t^{118}+2t^{117}+t^{116}+t^{115}+\\
&2t^{114}+2t^{113}+4t^{112}+2t^{111}+2t^{110}+t^{109}+t^{108}+2t^{107}+t^{106}+\\
&t^{105}+t^{104}+t^{103}+2t^{102}+t^{101}+t^{100}+t^{99}+t^{98}+2t^{97}+t^{96}+t^{95}+t^{94}+\\
&t^{93}+2t^{92}+t^{91}+t^{90}+2t^{89}+2t^{88}+4t^{87}+2t^{86}+2t^{85}+t^{84}+t^{83}+\\
&2t^{82}+t^{81}+t^{80}+t^{79}+t^{78}+2t^{77}+t^{76}+t^{75}+2t^{74}+2t^{73}+4t^{72}+2t^{71}+\\
&2t^{70}+2t^{69}+2t^{68}+4t^{67}+2t^{66}+2t^{65}+4t^{64}+4t^{63}+8t^{62}+4t^{61}+\\
&4t^{60}+2t^{59}+2t^{58}+4t^{57}+2t^{56}+2t^{55}+2t^{54}+2t^{53}+4t^{52}+2t^{51}+\\
&2t^{50}+t^{49}+t^{48}+2t^{47}+t^{46}+t^{45}+t^{44}+t^{43}+2t^{42}+t^{41}+t^{40}+2t^{39}+\\
&2t^{38}+4t^{37}+2t^{36}+2t^{35}+t^{34}+t^{33}+2t^{32}+t^{31}+t^{30}+t^{29}+t^{28}+2t^{27}+\\
&t^{26}+t^{25}+t^{24}+t^{23}+2t^{22}+t^{21}+t^{20}+t^{19}+t^{18}+2t^{17}+t^{16}+t^{15}+2t^{14}+\\
&2t^{13}+4t^{12}+2t^{11}+2t^{10}+t^9+t^8+2t^7+t^6+t^5+t^4+t^3+2t^2+t+1
\end{align*}

\begin{align*}
A_{21}[d;&125](t)=t^{124}+3t^{123}+90t^{122}+3183t^{121}+94261t^{120}+\\
&2253202t^{119}+44660548t^{118}+752765650t^{117}+11009028511t^{116}+\\
&141893733677t^{115}+1631777415270t^{114}+16911146129477t^{113}+\\
&159246625098675t^{112}+1371970915997752t^{111}+10877769405955360t^{110}+\\
&79770308934046652t^{109}+543435229636808801t^{108}+3452412046875069875t^{107}+\\
&20522671612161479218t^{106}+114494904782475069427t^{105}+\\
&601098250109024238421t^{104}+2976867524344065707158t^{103}+\\
&13937152500343124859524t^{102}+61808241523238164274278t^{101}+\\
&260109683076982063079271t^{100}+1040438732307841647264001t^{99}+\\
&3961670557633787552369622t^{98}+14379396838818630702670729t^{97}+\\
&49814339048764832456390627t^{96}+164902639609703309837818576t^{95}+\\
&522191692097394744372570064t^{94}+1583419969585645757298166644t^{93}+\\
&4601814286608285714581287637t^{92}+12829300435392788916008371659t^{91}+\\
&34337245282963060081957805954t^{90}+88295773584762135475767267735t^{89}+\\
&218286773584550853415117681033t^{88}+519168542579472256033947258058t^{87}+\\
&1188622715905633892159206423188t^{86}+2621065476099602847256268985110t^{85}+\\
&5569764136711656142481362767183t^{84}+11411224084970222152069566117509t^{83}+\\
&22550752358393534437025056773982t^{82}+43003760311355111831098813088769t^{81}+\\
&79166013300449183486759966707923t^{80}+140739579200798547810856736509576t^{79}+\\
&241704929497023593576293669675592t^{78}+401127329803571069200032815963604t^{77}+\\
&643475091559895257811487192086457t^{76}+998042999154123255509591723712251t^{75}+\\
&1497064498731184884738438067393274t^{74}+2172211233453091791403216937366843t^{73}+\\
&3049450385424532709259897590332593t^{72}+4142649580199365187088270983859398t^{71}+\\
&5446817040632498674709277300717412t^{70}+6932312597168634673342988991544262t^{69}+\\
&8541599450082782011722336731949035t^{68}+10189978291326827658936491765174825t^{67}+\\
&11771181819291335403215232033465030t^{66}+13167762713105561632909744695314237t^{65}+\\
&14265076272531025106827725830461707t^{64}+14966637400688288631941128601570312t^{63}+\\
&15208034778118744904852527054387840t^{62}+14966637400688288631941128601570312t^{61}+\\
&14265076272531025106827725830461707t^{60}+13167762713105561632909744695314237t^{59}+\\
&11771181819291335403215232033465030t^{58}+10189978291326827658936491765174825t^{57}+\\
\end{align*}
%A_21 continued
\begin{align*}
&8541599450082782011722336731949035t^{56}+6932312597168634673342988991544262t^{55}+\\
&5446817040632498674709277300717412t^{54}+4142649580199365187088270983859398t^{53}+\\
&3049450385424532709259897590332593t^{52}+2172211233453091791403216937366843t^{51}+\\
&1497064498731184884738438067393274t^{50}+998042999154123255509591723712251t^{49}+\\
&643475091559895257811487192086457t^{48}+401127329803571069200032815963604t^{47}+\\
&241704929497023593576293669675592t^{46}+140739579200798547810856736509576t^{45}+\\
&79166013300449183486759966707923t^{44}+43003760311355111831098813088769t^{43}+\\
&22550752358393534437025056773982t^{42}+11411224084970222152069566117509t^{41}+\\
&5569764136711656142481362767183t^{40}+2621065476099602847256268985110t^{39}+\\
&1188622715905633892159206423188t^{38}+519168542579472256033947258058t^{37}+\\
&218286773584550853415117681033t^{36}+88295773584762135475767267735t^{35}+\\
&34337245282963060081957805954t^{34}+12829300435392788916008371659t^{33}+\\
&4601814286608285714581287637t^{32}+1583419969585645757298166644t^{31}+\\
&522191692097394744372570064t^{30}+164902639609703309837818576t^{29}+\\
&49814339048764832456390627t^{28}+14379396838818630702670729t^{27}+\\
&3961670557633787552369622t^{26}+1040438732307841647264001t^{25}+\\
&260109683076982063079271t^{24}+61808241523238164274278t^{23}+\\
&13937152500343124859524t^{22}+2976867524344065707158t^{21}+\\
&601098250109024238421t^{20}+114494904782475069427t^{19}+\\
&20522671612161479218t^{18}+3452412046875069875t^{17}+\\
&543435229636808801t^{16}+79770308934046652t^{15}+10877769405955360t^{14}+\\
&1371970915997752t^{13}+159246625098675t^{12}+16911146129477t^{11}+\\
&1631777415270t^{10}+141893733677t^9+11009028511t^8+752765650t^7+\\
&44660548t^6+2253202t^5+94261t^4+3183t^3+90t^2+3t+1
\end{align*}


\begin{align*}
A_{22}[d;&125](t)=t^{124}+2t^{123}+16t^{122}+102t^{121}+536t^{120}+\\
&2127t^{119}+6768t^{118}+17586t^{117}+38827t^{116}+76002t^{115}+\\
&140618t^{114}+259636t^{113}+483996t^{112}+879511t^{111}+1506588t^{110}+\\
&2430477t^{109}+3813087t^{108}+6025186t^{107}+9605478t^{106}+\\
&14990352t^{105}+22363341t^{104}+32126727t^{103}+45830880t^{102}+\\
&66260127t^{101}+95776861t^{100}+134520876t^{99}+181894438t^{98}+\\
&241482810t^{97}+323296983t^{96}+437175501t^{95}+582695804t^{94}+\\
&751017303t^{93}+943649236t^{92}+1186422728t^{91}+1511709474t^{90}+\\
&1920090810t^{89}+2374236579t^{88}+2851940514t^{87}+3400809384t^{86}+\\
&4105791435t^{85}+4981822098t^{84}+5929999778t^{83}+6852264216t^{82}+\\
&7805305478t^{81}+8968682293t^{80}+10411728126t^{79}+11949925688t^{78}+\\
&13334526060t^{77}+14585287978t^{76}+16008752876t^{75}+17798416164t^{74}+\\
&19707130012t^{73}+21283301536t^{72}+22438886362t^{71}+23596306968t^{70}+\\
&25139780062t^{69}+26846406914t^{68}+28090065316t^{67}+28621603364t^{66}+\\
&28906040812t^{65}+29522002718t^{64}+30378601066t^{63}+30797103792t^{62}+\\
&30378601066t^{61}+29522002718t^{60}+28906040812t^{59}+28621603364t^{58}+\\
&28090065316t^{57}+26846406914t^{56}+25139780062t^{55}+23596306968t^{54}+\\
&22438886362t^{53}+21283301536t^{52}+19707130012t^{51}+17798416164t^{50}+\\
&16008752876t^{49}+14585287978t^{48}+13334526060t^{47}+11949925688t^{46}+\\
&10411728126t^{45}+8968682293t^{44}+7805305478t^{43}+6852264216t^{42}+\\
&5929999778t^{41}+4981822098t^{40}+4105791435t^{39}+3400809384t^{38}+\\
&2851940514t^{37}+2374236579t^{36}+1920090810t^{35}+1511709474t^{34}+\\
&1186422728t^{33}+943649236t^{32}+751017303t^{31}+582695804t^{30}+\\
&437175501t^{29}+323296983t^{28}+241482810t^{27}+181894438t^{26}+\\
&134520876t^{25}+95776861t^{24}+66260127t^{23}+45830880t^{22}+\\
&32126727t^{21}+22363341t^{20}+14990352t^{19}+9605478t^{18}+\\
&6025186t^{17}+3813087t^{16}+2430477t^{15}+1506588t^{14}+879511t^{13}+\\
&483996t^{12}+259636t^{11}+140618t^{10}+76002t^9+38827t^8+17586t^7+\\
&6768t^6+2127t^5+536t^4+102t^3+16t^2+2t+1
\end{align*}

\begin{align*}
A_{2}[d;&125](t)=t^{123}+74t^{122}+3081t^{121}+93725t^{120}+2251075t^{119}+\\
&44653780t^{118}+752748064t^{117}+11008989684t^{116}+141893657675t^{115}+\\
&1631777274652t^{114}+16911145869841t^{113}+159246624614679t^{112}+\\
&1371970915118241t^{111}+10877769404448772t^{110}+79770308931616175t^{109}+\\
&543435229632995714t^{108}+3452412046869044689t^{107}+\\
&20522671612151873740t^{106}+114494904782460079075t^{105}+\\
&601098250109001875080t^{104}+2976867524344033580431t^{103}+\\
&13937152500343079028644t^{102}+61808241523238098014151t^{101}+\\
&260109683076981967302410t^{100}+1040438732307841512743125t^{99}+\\
&3961670557633787370475184t^{98}+14379396838818630461187919t^{97}+\\
&49814339048764832133093644t^{96}+164902639609703309400643075t^{95}+\\
&522191692097394743789874260t^{94}+1583419969585645756547149341t^{93}+\\
&4601814286608285713637638401t^{92}+12829300435392788914821948931t^{91}+\\
&34337245282963060080446096480t^{90}+88295773584762135473847176925t^{89}+\\
&218286773584550853412743444454t^{88}+519168542579472256031095317544t^{87}+\\
&1188622715905633892155805613804t^{86}+2621065476099602847252163193675t^{85}+\\
&5569764136711656142476380945085t^{84}+11411224084970222152063636117731t^{83}+\\
&22550752358393534437018204509766t^{82}+43003760311355111831091007783291t^{81}+\\
&79166013300449183486750998025630t^{80}+140739579200798547810846324781450t^{79}+\\
&241704929497023593576281719749904t^{78}+401127329803571069200019481437544t^{77}+\\
&643475091559895257811472606798479t^{76}+998042999154123255509575714959375t^{75}+\\
&1497064498731184884738420268977110t^{74}+2172211233453091791403197230236831t^{73}+\\
&3049450385424532709259876307031057t^{72}+4142649580199365187088248544973036t^{71}+\\
&5446817040632498674709253704410444t^{70}+6932312597168634673342963851764200t^{69}+\\
&8541599450082782011722309885542121t^{68}+10189978291326827658936463675109509t^{67}+\\
&11771181819291335403215203411861666t^{66}+13167762713105561632909715789273425t^{65}+\\
&14265076272531025106827696308458989t^{64}+14966637400688288631941098222969246t^{63}+\\
&15208034778118744904852496257284048t^{62}+14966637400688288631941098222969246t^{61}+\\
&14265076272531025106827696308458989t^{60}+13167762713105561632909715789273425t^{59}+\\
&11771181819291335403215203411861666t^{58}+10189978291326827658936463675109509t^{57}+\\
\end{align*}
%A_2 continued
\begin{align*}
A_{2}[d;&125](t)continued...\\
&8541599450082782011722309885542121t^{56}+6932312597168634673342963851764200t^{55}+\\
&5446817040632498674709253704410444t^{54}+4142649580199365187088248544973036t^{53}+\\
&3049450385424532709259876307031057t^{52}+2172211233453091791403197230236831t^{51}+\\
&1497064498731184884738420268977110t^{50}+998042999154123255509575714959375t^{49}+\\
&643475091559895257811472606798479t^{48}+401127329803571069200019481437544t^{47}+\\
&241704929497023593576281719749904t^{46}+140739579200798547810846324781450t^{45}+\\
&79166013300449183486750998025630t^{44}+43003760311355111831091007783291t^{43}+\\
&22550752358393534437018204509766t^{42}+11411224084970222152063636117731t^{41}+\\
&5569764136711656142476380945085t^{40}+2621065476099602847252163193675t^{39}+\\
&1188622715905633892155805613804t^{38}+519168542579472256031095317544t^{37}+\\
&218286773584550853412743444454t^{36}+88295773584762135473847176925t^{35}+\\
&34337245282963060080446096480t^{34}+12829300435392788914821948931t^{33}+\\
&4601814286608285713637638401t^{32}+1583419969585645756547149341t^{31}+\\
&522191692097394743789874260t^{30}+164902639609703309400643075t^{29}+\\
&49814339048764832133093644t^{28}+14379396838818630461187919t^{27}+\\
&3961670557633787370475184t^{26}+1040438732307841512743125t^{25}+\\
&260109683076981967302410t^{24}+61808241523238098014151t^{23}+13937152500343079028644t^{22}+\\
&2976867524344033580431t^{21}+601098250109001875080t^{20}+114494904782460079075t^{19}+\\
&20522671612151873740t^{18}+3452412046869044689t^{17}+543435229632995714t^{16}+\\
&79770308931616175t^{15}+10877769404448772t^{14}+1371970915118241t^{13}+\\
&159246624614679t^{12}+16911145869841t^{11}+1631777274652t^{10}+141893657675t^{9}+\\
&11008989684t^8+752748064t^7+44653780t^6+2251075t^5+93725t^4+3081t^3+74t^2+t
\end{align*}


\begin{align*}
A_{31}[d;&125](t)=t^{124}+t^{123}+2t^{122}+t^{121}+t^{120}+2t^{119}+2t^{118}+\\
&4t^{117}+2t^{116}+2t^{115}+16t^{114}+16t^{113}+32t^{112}+16t^{111}+16t^{110}+\\
&102t^{109}+102t^{108}+204t^{107}+102t^{106}+102t^{105}+536t^{104}+536t^{103}+\\
&1072t^{102}+536t^{101}+536t^{100}+2126t^{99}+2126t^{98}+4252t^{97}+2126t^{96}+\\
&2126t^{95}+6744t^{94}+6744t^{93}+13488t^{92}+6744t^{91}+6744t^{90}+17310t^{89}+\\
&17310t^{88}+34620t^{87}+17310t^{86}+17310t^{85}+36803t^{84}+36803t^{83}+\\
&73606t^{82}+36803t^{81}+36803t^{80}+65376t^{79}+65376t^{78}+130752t^{77}+\\
&65376t^{76}+65376t^{75}+98104t^{74}+98104t^{73}+196208t^{72}+98104t^{71}+\\
&98104t^{70}+124812t^{69}+124812t^{68}+249624t^{67}+124812t^{66}+124812t^{65}+\\
&135264t^{64}+135264t^{63}+270528t^{62}+135264t^{61}+135264t^{60}+124812t^{59}+\\
&124812t^{58}+249624t^{57}+124812t^{56}+124812t^{55}+98104t^{54}+98104t^{53}+\\
&196208t^{52}+98104t^{51}+98104t^{50}+65376t^{49}+65376t^{48}+130752t^{47}+\\
&65376t^{46}+65376t^{45}+36803t^{44}+36803t^{43}+73606t^{42}+36803t^{41}+\\
&36803t^{40}+17310t^{39}+17310t^{38}+34620t^{37}+17310t^{36}+17310t^{35}+\\
&6744t^{34}+6744t^{33}+13488t^{32}+6744t^{31}+6744t^{30}+2126t^{29}+2126t^{28}+\\
&4252t^{27}+2126t^{26}+2126t^{25}+536t^{24}+536t^{23}+1072t^{22}+536t^{21}+\\
&536t^{20}+102t^{19}+102t^{18}+204t^{17}+102t^{16}+102t^{15}+16t^{14}+16t^{13}+\\
&32t^{12}+16t^{11}+16t^{10}+2t^9+2t^8+4t^7+2t^6+2t^5+t^4+t^3+2t^2+t+1\\
\end{align*}

\begin{align*}
A_{32}[d;&125](t)=t^{124}+t^{123}+2t^{122}+t^{121}+t^{120}+t^{119}+t^{118}+2t^{117}+t^{116}+\\
&t^{115}+2t^{114}+2t^{113}+4t^{112}+2t^{111}+2t^{110}+t^{109}+t^{108}+2t^{107}+t^{106}+t^{105}+\\
&t^{104}+t^{103}+2t^{102}+t^{101}+t^{100}+t^{99}+t^{98}+2t^{97}+t^{96}+t^{95}+4t^{94}+4t^{93}+8t^{92}+\\
&4t^{91}+4t^{90}+6t^{89}+6t^{88}+12t^{87}+6t^{86}+6t^{85}+4t^{84}+4t^{83}+8t^{82}+4t^{81}+\\
&4t^{80}+t^{79}+t^{78}+2t^{77}+t^{76}+t^{75}+2t^{74}+2t^{73}+4t^{72}+2t^{71}+2t^{70}+6t^{69}+\\
&6t^{68}+12t^{67}+6t^{66}+6t^{65}+10t^{64}+10t^{63}+20t^{62}+10t^{61}+10t^{60}+6t^{59}+\\
&6t^{58}+12t^{57}+6t^{56}+6t^{55}+2t^{54}+2t^{53}+4t^{52}+2t^{51}+2t^{50}+t^{49}+t^{48}+2t^{47}+\\
&t^{46}+t^{45}+4t^{44}+4t^{43}+8t^{42}+4t^{41}+4t^{40}+6t^{39}+6t^{38}+12t^{37}+6t^{36}+6t^{35}+\\
&4t^{34}+4t^{33}+8t^{32}+4t^{31}+4t^{30}+t^{29}+t^{28}+2t^{27}+t^{26}+t^{25}+t^{24}+t^{23}+2t^{22}+t^{21}+\\
&t^{20}+t^{19}+t^{18}+2t^{17}+t^{16}+t^{15}+2t^{14}+2t^{13}+4t^{12}+2t^{11}+2t^{10}+t^9+t^8+2t^7+t^6+\\
&t^5+t^4+t^3+2t^2+t+1
\end{align*}

\begin{align*}
A_{3}&[d;125](t)=t^{119}+t^{118}+2t^{117}+t^{116}+t^{115}+14t^{114}+14t^{113}+28t^{112}+14t^{111}+\\
&14t^{110}+101t^{109}+101t^{108}+202t^{107}+101t^{106}+101t^{105}+535t^{104}+535t^{103}+1070t^{102}+\\
&535t^{101}+535t^{100}+2125t^{99}+2125t^{98}+4250t^{97}+2125t^{96}+2125t^{95}+6740t^{94}+6740t^{93}+\\
&13480t^{92}+6740t^{91}+6740t^{90}+17304t^{89}+17304t^{88}+34608t^{87}+17304t^{86}+17304t^{85}+\\
&36799t^{84}+36799t^{83}+73598t^{82}+36799t^{81}+36799t^{80}+65375t^{79}+65375t^{78}+130750t^{77}+\\
&65375t^{76}+65375t^{75}+98102t^{74}+98102t^{73}+196204t^{72}+98102t^{71}+98102t^{70}+124806t^{69}+\\
&124806t^{68}+249612t^{67}+124806t^{66}+124806t^{65}+135254t^{64}+135254t^{63}+270508t^{62}+\\
&135254t^{61}+135254t^{60}+124806t^{59}+124806t^{58}+249612t^{57}+124806t^{56}+\\
&124806t^{55}+98102t^{54}+98102t^{53}+196204t^{52}+98102t^{51}+98102t^{50}+65375t^{49}+65375t^{48}+\\
&130750t^{47}+65375t^{46}+65375t^{45}+36799t^{44}+36799t^{43}+73598t^{42}+36799t^{41}+36799t^{40}+\\
&17304t^{39}+17304t^{38}+34608t^{37}+17304t^{36}+17304t^{35}+6740t^{34}+6740t^{33}+13480t^{32}+\\
&6740t^{31}+6740t^{30}+2125t^{29}+2125t^{28}+4250t^{27}+2125t^{26}+2125t^{25}+535t^{24}+535t^{23}+\\
&1070t^{22}+535t^{21}+535t^{20}+101t^{19}+101t^{18}+202t^{17}+101t^{16}+101t^{15}+14t^{14}+14t^{13}+\\
&28t^{12}+14t^{11}+14t^{10}+t^9+t^8+2t^7+t^6+t^5
\end{align*}

\begin{align*}
A_{41}[d;&125](t)=t^{124}+2t^{123}+16t^{122}+102t^{121}+536t^{120}+2126t^{119}+6744t^{118}+\\
&17310t^{117}+36803t^{116}+65376t^{115}+98104t^{114}+124812t^{113}+135264t^{112}+124812t^{111}+\\
&98104t^{110}+65376t^{109}+36803t^{108}+17310t^{107}+6744t^{106}+2126t^{105}+536t^{104}+\\
&102t^{103}+16t^{102}+2t^{101}+t^{100}+t^{99}+2t^{98}+16t^{97}+102t^{96}+536t^{95}+2126t^{94}+\\
&6744t^{93}+17310t^{92}+36803t^{91}+65376t^{90}+98104t^{89}+124812t^{88}+135264t^{87}+\\
&124812t^{86}+98104t^{85}+65376t^{84}+36803t^{83}+17310t^{82}+6744t^{81}+2126t^{80}+536t^{79}+\\
&102t^{78}+16t^{77}+2t^{76}+t^{75}+2t^{74}+4t^{73}+32t^{72}+204t^{71}+1072t^{70}+4252t^{69}+\\
&13488t^{68}+34620t^{67}+73606t^{66}+130752t^{65}+196208t^{64}+249624t^{63}+270528t^{62}+\\
&249624t^{61}+196208t^{60}+130752t^{59}+73606t^{58}+34620t^{57}+13488t^{56}+4252t^{55}+1072t^{54}+\\
&204t^{53}+32t^{52}+4t^{51}+2t^{50}+t^{49}+2t^{48}+16t^{47}+102t^{46}+536t^{45}+2126t^{44}+\\
&6744t^{43}+17310t^{42}+36803t^{41}+65376t^{40}+98104t^{39}+124812t^{38}+135264t^{37}+124812t^{36}+\\
&98104t^{35}+65376t^{34}+36803t^{33}+17310t^{32}+6744t^{31}+2126t^{30}+536t^{29}+102t^{28}+16t^{27}+\\
&2t^{26}+t^{25}+t^{24}+2t^{23}+16t^{22}+102t^{21}+536t^{20}+2126t^{19}+6744t^{18}+\\
&17310t^{17}+36803t^{16}+65376t^{15}+98104t^{14}+124812t^{13}+135264t^{12}+124812t^{11}+\\
&98104t^{10}+65376t^9+36803t^8+17310t^7+6744t^6+2126t^5+536t^4+102t^3+16t^2+2t+1\\
\end{align*}

\begin{align*}
A_{42}[d;&125](t)=t^{124}+t^{123}+2t^{122}+t^{121}+t^{120}+t^{119}+4t^{118}+6t^{117}+4t^{116}+\\
&t^{115}+2t^{114}+6t^{113}+10t^{112}+6t^{111}+2t^{110}+t^{109}+4t^{108}+6t^{107}+4t^{106}+t^{105}+\\
&t^{104}+t^{103}+2t^{102}+t^{101}+t^{100}+t^{99}+t^{98}+2t^{97}+t^{96}+t^{95}+t^{94}+4t^{93}+6t^{92}+\\
&4t^{91}+t^{90}+2t^{89}+6t^{88}+10t^{87}+6t^{86}+2t^{85}+t^{84}+4t^{83}+6t^{82}+4t^{81}+t^{80}+t^{79}+\\
&t^{78}+2t^{77}+t^{76}+t^{75}+2t^{74}+2t^{73}+4t^{72}+2t^{71}+2t^{70}+2t^{69}+8t^{68}+12t^{67}+8t^{66}+\\
&2t^{65}+4t^{64}+12t^{63}+20t^{62}+12t^{61}+4t^{60}+2t^{59}+8t^{58}+12t^{57}+8t^{56}+2t^{55}+2t^{54}+\\
&2t^{53}+4t^{52}+2t^{51}+2t^{50}+t^{49}+t^{48}+2t^{47}+t^{46}+t^{45}+t^{44}+4t^{43}+6t^{42}+4t^{41}+\\
&t^{40}+2t^{39}+6t^{38}+10t^{37}+6t^{36}+2t^{35}+t^{34}+4t^{33}+6t^{32}+4t^{31}+t^{30}+t^{29}+t^{28}+\\
&2t^{27}+t^{26}+t^{25}+t^{24}+t^{23}+2t^{22}+t^{21}+t^{20}+t^{19}+4t^{18}+6t^{17}+4t^{16}+t^{15}+2t^{14}+\\
&6t^{13}+10t^{12}+6t^{11}+2t^{10}+t^9+4t^8+6t^7+4t^6+t^5+t^4+t^3+2t^2+t+1
\end{align*}

\begin{align*}
A_{4}[d;&125](t)=t^{123}+14t^{122}+101t^{121}+535t^{120}+2125t^{119}+6740t^{118}+17304t^{117}+\\
&36799t^{116}+65375t^{115}+98102t^{114}+124806t^{113}+135254t^{112}+124806t^{111}+98102t^{110}+\\
&65375t^{109}+36799t^{108}+17304t^{107}+6740t^{106}+2125t^{105}+535t^{104}+101t^{103}+14t^{102}+\\
&t^{101}+t^{98}+14t^{97}+101t^{96}+535t^{95}+2125t^{94}+6740t^{93}+17304t^{92}+36799t^{91}+\\
&65375t^{90}+98102t^{89}+124806t^{88}+135254t^{87}+124806t^{86}+98102t^{85}+65375t^{84}+\\
&36799t^{83}+17304t^{82}+6740t^{81}+2125t^{80}+535t^{79}+101t^{78}+14t^{77}+t^{76}+2t^{73}+\\
&28t^{72}+202t^{71}+1070t^{70}+4250t^{69}+13480t^{68}+34608t^{67}+73598t^{66}+130750t^{65}+\\
&196204t^{64}+249612t^{63}+270508t^{62}+249612t^{61}+196204t^{60}+130750t^{59}+73598t^{58}+\\
&34608t^{57}+13480t^{56}+4250t^{55}+1070t^{54}+202t^{53}+28t^{52}+2t^{51}+t^{48}+14t^{47}+\\
&101t^{46}+535t^{45}+2125t^{44}+6740t^{43}+17304t^{42}+36799t^{41}+65375t^{40}+98102t^{39}+\\
&124806t^{38}+135254t^{37}+124806t^{36}+98102t^{35}+65375t^{34}+36799t^{33}+17304t^{32}+\\
&6740t^{31}+2125t^{30}+535t^{29}+101t^{28}+14t^{27}+t^{26}+t^{23}+14t^{22}+101t^{21}+\\
&535t^{20}+2125t^{19}+6740t^{18}+17304t^{17}+36799t^{16}+65375t^{15}+98102t^{14}+124806t^{13}+\\
&135254t^{12}+124806t^{11}+98102t^{10}+65375t^{9}+36799t^{8}+17304t^{7}+6740t^6+2125t^5+\\
&535t^4+101t^3+14t^2+t
\end{align*}

\begin{align*}
A_{51}[d;&125](t)=t^{124}+2t^{123}+16t^{122}+102t^{121}+536t^{120}+2127t^{119}+6752t^{118}+17370t^{117}+\\
&37211t^{116}+67502t^{115}+106618t^{114}+151820t^{113}+205076t^{112}+275795t^{111}+379812t^{110}+\\
&538477t^{109}+792383t^{108}+1219370t^{107}+1926814t^{106}+2999852t^{105}+4473525t^{104}+\\
&6427127t^{103}+9168744t^{102}+13253727t^{101}+19155801t^{100}+26905876t^{99}+36385694t^{98}+\\
&48306810t^{97}+64666523t^{96}+87438501t^{95}+116551356t^{94}+150246539t^{93}+188817556t^{92}+\\
&237423764t^{91}+302556490t^{90}+384345810t^{89}+475302087t^{88}+570903850t^{87}+\\
&680616648t^{86}+821485935t^{85}+996603062t^{84}+1186235314t^{83}+1370684784t^{82}+\\
&1561200314t^{81}+1793772701t^{80}+2082399626t^{79}+2390194664t^{78}+2667219060t^{77}+\\
&2917266802t^{76}+3201802876t^{75}+3559761716t^{74}+3941739812t^{73}+4257131144t^{72}+\\
&4488091562t^{71}+4719342432t^{70}+5028066062t^{69}+5369713098t^{68}+5618695220t^{67}+\\
&5724896620t^{66}+5781621812t^{65}+5904979518t^{64}+6076751970t^{63}+6160718928t^{62}+\\
&6076751970t^{61}+5904979518t^{60}+5781621812t^{59}+5724896620t^{58}+5618695220t^{57}+\\
&5369713098t^{56}+5028066062t^{55}+4719342432t^{54}+4488091562t^{53}+4257131144t^{52}+\\
&3941739812t^{51}+3559761716t^{50}+3201802876t^{49}+2917266802t^{48}+2667219060t^{47}+\\
&2390194664t^{46}+2082399626t^{45}+1793772701t^{44}+1561200314t^{43}+1370684784t^{42}+\\
&1186235314t^{41}+996603062t^{40}+821485935t^{39}+680616648t^{38}+570903850t^{37}+\\
&475302087t^{36}+384345810t^{35}+302556490t^{34}+237423764t^{33}+188817556t^{32}+\\
&150246539t^{31}+116551356t^{30}+87438501t^{29}+64666523t^{28}+48306810t^{27}+36385694t^{26}+\\
&26905876t^{25}+19155801t^{24}+13253727t^{23}+9168744t^{22}+6427127t^{21}+4473525t^{20}+\\
&2999852t^{19}+1926814t^{18}+1219370t^{17}+792383t^{16}+538477t^{15}+379812t^{14}+\\
&275795t^{13}+205076t^{12}+151820t^{11}+106618t^{10}+67502t^9+37211t^8+17370t^7+6752t^6+\\
&2127t^5+536t^4+102t^3+16t^2+2t+1
\end{align*}

\begin{align*}
A5_{21}[d;&125](t)=t^{124}+2t^{123}+16t^{122}+102t^{121}+536t^{120}+2126t^{119}+\\
&6744t^{118}+17310t^{117}+36803t^{116}+65376t^{115}+98104t^{114}+124812t^{113}+\\
&135264t^{112}+124812t^{111}+98104t^{110}+65376t^{109}+36803t^{108}+17310t^{107}+\\
&6744t^{106}+2126t^{105}+536t^{104}+102t^{103}+16t^{102}+2t^{101}+t^{100}+t^{99}+\\
&8t^{98}+60t^{97}+408t^{96}+2126t^{95}+8504t^{94}+26932t^{93}+69240t^{92}+\\
&147107t^{91}+261504t^{90}+392256t^{89}+499248t^{88}+540860t^{87}+\\
&499248t^{86}+392256t^{85}+261504t^{84}+147107t^{83}+69240t^{82}+26932t^{81}+\\
&8504t^{80}+2126t^{79}+408t^{78}+60t^{77}+8t^{76}+t^{75}+2t^{74}+12t^{73}+92t^{72}+\\
&612t^{71}+3196t^{70}+12756t^{69}+40420t^{68}+103860t^{67}+220710t^{66}+392256t^{65}+\\
&588464t^{64}+748872t^{63}+811384t^{62}+748872t^{61}+588464t^{60}+392256t^{59}+\\
&220710t^{58}+103860t^{57}+40420t^{56}+12756t^{55}+3196t^{54}+612t^{53}+92t^{52}+\\
&12t^{51}+2t^{50}+t^{49}+8t^{48}+60t^{47}+408t^{46}+2126t^{45}+8504t^{44}+\\
&26932t^{43}+69240t^{42}+147107t^{41}+261504t^{40}+392256t^{39}+499248t^{38}+\\
&540860t^{37}+499248t^{36}+392256t^{35}+261504t^{34}+147107t^{33}+69240t^{32}+\\
&26932t^{31}+8504t^{30}+2126t^{29}+408t^{28}+60t^{27}+8t^{26}+t^{25}+t^{24}+\\
&2t^{23}+16t^{22}+102t^{21}+536t^{20}+2126t^{19}+6744t^{18}+17310t^{17}+\\
&36803t^{16}+65376t^{15}+98104t^{14}+124812t^{13}+135264t^{12}+124812t^{11}+\\
&98104t^{10}+65376t^9+36803t^8+17310t^7+6744t^6+2126t^5+536t^4+102t^3+16t^2+2t+1\\
\end{align*}


\begin{align*}
A5_{22}[d;&125](t)=t^{124}+t^{123}+2t^{122}+t^{121}+t^{120}+2t^{119}+\\
&8t^{118}+12t^{117}+8t^{116}+2t^{115}+16t^{114}+60t^{113}+92t^{112}+60t^{111}+\\
&16t^{110}+102t^{109}+408t^{108}+612t^{107}+408t^{106}+102t^{105}+536t^{104}+\\
&2126t^{103}+3196t^{102}+2126t^{101}+536t^{100}+2126t^{99}+8504t^{98}+12756t^{97}+\\
&8504t^{96}+2126t^{95}+6744t^{94}+26932t^{93}+40420t^{92}+26932t^{91}+6744t^{90}+\\
&17310t^{89}+69240t^{88}+103860t^{87}+69240t^{86}+17310t^{85}+36803t^{84}+\\
&147107t^{83}+220710t^{82}+147107t^{81}+36803t^{80}+65376t^{79}+\\
&261504t^{78}+392256t^{77}+261504t^{76}+65376t^{75}+98104t^{74}+\\
&392256t^{73}+588464t^{72}+392256t^{71}+98104t^{70}+124812t^{69}+499248t^{68}+\\
&748872t^{67}+499248t^{66}+124812t^{65}+135264t^{64}+540860t^{63}+811384t^{62}+\\
&540860t^{61}+135264t^{60}+124812t^{59}+499248t^{58}+748872t^{57}+499248t^{56}+\\
&124812t^{55}+98104t^{54}+392256t^{53}+588464t^{52}+392256t^{51}+98104t^{50}+\\
&65376t^{49}+261504t^{48}+392256t^{47}+261504t^{46}+65376t^{45}+36803t^{44}+\\
&147107t^{43}+220710t^{42}+147107t^{41}+36803t^{40}+17310t^{39}+69240t^{38}+\\
&103860t^{37}+69240t^{36}+17310t^{35}+6744t^{34}+26932t^{33}+40420t^{32}+\\
&26932t^{31}+6744t^{30}+2126t^{29}+8504t^{28}+12756t^{27}+8504t^{26}+2126t^{25}+\\
&536t^{24}+2126t^{23}+3196t^{22}+2126t^{21}+536t^{20}+102t^{19}+408t^{18}+\\
&612t^{17}+408t^{16}+102t^{15}+16t^{14}+60t^{13}+92t^{12}+60t^{11}+16t^{10}+2t^9+\\
&8t^8+12t^7+8t^6+2t^5+t^4+t^3+2t^2+t+1\\
\end{align*}

\begin{align*}
A5_{23}[d;&125](t)=t^{124}+t^{123}+2t^{122}+t^{121}+t^{120}+t^{119}+4t^{118}+\\
&6t^{117}+4t^{116}+t^{115}+2t^{114}+6t^{113}+10t^{112}+6t^{111}+2t^{110}+t^{109}+\\
&4t^{108}+6t^{107}+4t^{106}+t^{105}+t^{104}+t^{103}+2t^{102}+t^{101}+t^{100}+\\
&t^{99}+4t^{98}+6t^{97}+4t^{96}+t^{95}+4t^{94}+16t^{93}+24t^{92}+16t^{91}+4t^{90}+\\
&6t^{89}+24t^{88}+36t^{87}+24t^{86}+6t^{85}+4t^{84}+16t^{83}+24t^{82}+16t^{81}+\\
&4t^{80}+t^{79}+4t^{78}+6t^{77}+4t^{76}+t^{75}+2t^{74}+6t^{73}+10t^{72}+6t^{71}+\\
&2t^{70}+6t^{69}+24t^{68}+36t^{67}+24t^{66}+6t^{65}+10t^{64}+36t^{63}+56t^{62}+\\
&36t^{61}+10t^{60}+6t^{59}+24t^{58}+36t^{57}+24t^{56}+6t^{55}+2t^{54}+6t^{53}+\\
&10t^{52}+6t^{51}+2t^{50}+t^{49}+4t^{48}+6t^{47}+4t^{46}+t^{45}+4t^{44}+16t^{43}+\\
&24t^{42}+16t^{41}+4t^{40}+6t^{39}+24t^{38}+36t^{37}+24t^{36}+6t^{35}+4t^{34}+\\
&16t^{33}+24t^{32}+16t^{31}+4t^{30}+t^{29}+4t^{28}+6t^{27}+4t^{26}+t^{25}+t^{24}+\\
&t^{23}+2t^{22}+t^{21}+t^{20}+t^{19}+4t^{18}+6t^{17}+4t^{16}+t^{15}+2t^{14}+6t^{13}+\\
&10t^{12}+6t^{11}+2t^{10}+t^9+4t^8+6t^7+4t^6+t^5+t^4+t^3+2t^2+t+1
\end{align*}

\begin{align*}
A_{52}[d;&125](t)=t^{124}+2t^{123}+16t^{122}+102t^{121}+536t^{120}+2127t^{119}+\\
&6748t^{118}+17316t^{117}+36807t^{116}+65377t^{115}+98118t^{114}+124866t^{113}+\\
&135346t^{112}+124866t^{111}+98118t^{110}+65477t^{109}+37207t^{108}+17916t^{107}+\\
&7148t^{106}+2227t^{105}+1071t^{104}+2227t^{103}+3210t^{102}+2127t^{101}+536t^{100}+\\
&2126t^{99}+8508t^{98}+12810t^{97}+8908t^{96}+4251t^{95}+15244t^{94}+53848t^{93}+\\
&109636t^{92}+174023t^{91}+268244t^{90}+409560t^{89}+568464t^{88}+644684t^{87}+\\
&568464t^{86}+409560t^{85}+298303t^{84}+294198t^{83}+289926t^{82}+174023t^{81}+\\
&45303t^{80}+67501t^{79}+261908t^{78}+392310t^{77}+261508t^{76}+65376t^{75}+\\
&98104t^{74}+392262t^{73}+588546t^{72}+392862t^{71}+101298t^{70}+137562t^{69}+\\
&539644t^{68}+852696t^{67}+719934t^{66}+517062t^{65}+723718t^{64}+1289696t^{63}+\\
&1622712t^{62}+1289696t^{61}+723718t^{60}+517062t^{59}+719934t^{58}+852696t^{57}+\\
&539644t^{56}+137562t^{55}+101298t^{54}+392862t^{53}+588546t^{52}+392262t^{51}+\\
&98104t^{50}+65376t^{49}+261508t^{48}+392310t^{47}+261908t^{46}+67501t^{45}+\\
&45303t^{44}+174023t^{43}+289926t^{42}+294198t^{41}+298303t^{40}+409560t^{39}+\\
&568464t^{38}+644684t^{37}+568464t^{36}+409560t^{35}+268244t^{34}+174023t^{33}+\\
&109636t^{32}+53848t^{31}+15244t^{30}+4251t^{29}+8908t^{28}+12810t^{27}+8508t^{26}+\\
&2126t^{25}+536t^{24}+2127t^{23}+3210t^{22}+2227t^{21}+1071t^{20}+2227t^{19}+\\
&7148t^{18}+17916t^{17}+37207t^{16}+65477t^{15}+98118t^{14}+124866t^{13}+\\
&135346t^{12}+124866t^{11}+98118t^{10}+65377t^9+36807t^8+17316t^7+6748t^6+\\
&2127t^5+536t^4+102t^3+16t^2+2t+1
\end{align*}

\begin{align*}
A_{5}[d;&125](t)=4t^{118}+54t^{117}+404t^{116}+2125t^{115}+8500t^{114}+\\
&26954t^{113}+69730t^{112}+150929t^{111}+281694t^{110}+473000t^{109}+\\
&755176t^{108}+1201454t^{107}+1919666t^{106}+2997625t^{105}+4472454t^{104}+\\
&6424900t^{103}+9165534t^{102}+13251600t^{101}+19155265t^{100}+26903750t^{99}+\\
&36377186t^{98}+48294000t^{97}+64657615t^{96}+87434250t^{95}+116536112t^{94}+\\
&150192691t^{93}+188707920t^{92}+237249741t^{91}+302288246t^{90}+\\
&383936250t^{89}+474733623t^{88}+570259166t^{87}+680048184t^{86}+821076375t^{85}+\\
&996304759t^{84}+1185941116t^{83}+1370394858t^{82}+1561026291t^{81}+\\
&1793727398t^{80}+2082332125t^{79}+2389932756t^{78}+2666826750t^{77}+\\
&2917005294t^{76}+3201737500t^{75}+3559663612t^{74}+3941347550t^{73}+\\
&4256542598t^{72}+4487698700t^{71}+4719241134t^{70}+5027928500t^{69}+\\
&5369173454t^{68}+5617842524t^{67}+5724176686t^{66}+5781104750t^{65}+\\
&5904255800t^{64}+6075462274t^{63}+6159096216t^{62}+6075462274t^{61}+\\
&5904255800t^{60}+5781104750t^{59}+5724176686t^{58}+5617842524t^{57}+\\
&5369173454t^{56}+5027928500t^{55}+4719241134t^{54}+4487698700t^{53}+\\
&4256542598t^{52}+3941347550t^{51}+3559663612t^{50}+3201737500t^{49}+\\
&2917005294t^{48}+2666826750t^{47}+2389932756t^{46}+2082332125t^{45}+\\
&1793727398t^{44}+1561026291t^{43}+1370394858t^{42}+1185941116t^{41}+\\
&996304759t^{40}+821076375t^{39}+680048184t^{38}+570259166t^{37}+\\
&474733623t^{36}+383936250t^{35}+302288246t^{34}+237249741t^{33}+\\
&188707920t^{32}+150192691t^{31}+116536112t^{30}+87434250t^{29}+\\
&64657615t^{28}+48294000t^{27}+36377186t^{26}+26903750t^{25}+\\
&19155265t^{24}+13251600t^{23}+9165534t^{22}+6424900t^{21}+\\
&4472454t^{20}+2997625t^{19}+1919666t^{18}+1201454t^{17}+755176t^{16}+\\
&473000t^{15}+281694t^{14}+150929t^{13}+69730t^{12}+26954t^{11}+\\
&8500t^{10}+2125t^9+404t^8+54t^7+4t^6
\end{align*}

\begin{align*}
Total&[d;125](t)=A_{1}+A_{2}+A_{3}+A_{4}+A_{5}\\
&t^{124}+3t^{123}+90t^{122}+3183t^{121}+94261t^{120}+2253202t^{119}+\\
&44660526t^{118}+752765426t^{117}+11009026889t^{116}+141893725177t^{115}+\\
&1631777381270t^{114}+16911146021617t^{113}+159246624819695t^{112}+\\
&1371970915393992t^{111}+10877769404828584t^{110}+79770308932154652t^{109}+\\
&543435229633787791t^{108}+3452412046870263651t^{107}+\\
&20522671612153800248t^{106}+114494904782463078927t^{105}+\\
&601098250109006348605t^{104}+2976867524344040005968t^{103}+\\
&13937152500343088195264t^{102}+61808241523238111266288t^{101}+\\
&260109683076981986458211t^{100}+1040438732307841539649001t^{99}+\\
&3961670557633787406854497t^{98}+14379396838818630509486185t^{97}+\\
&49814339048764832197753486t^{96}+164902639609703309488079986t^{95}+\\
&522191692097394743906419238t^{94}+1583419969585645756697355513t^{93}+\\
&4601814286608285713826377107t^{92}+12829300435392788915059242212t^{91}+\\
&34337245282963060080748456842t^{90}+88295773584762135474231228583t^{89}+\\
&218286773584550853413218320189t^{88}+519168542579472256031665746576t^{87}+\\
&1188622715905633892156485804100t^{86}+2621065476099602847252984385458t^{85}+\\
&5569764136711656142477377352019t^{84}+11411224084970222152064822132446t^{83}+\\
&22550752358393534437019574995528t^{82}+43003760311355111831092568853122t^{81}+\\
&79166013300449183486752791791953t^{80}+140739579200798547810848407179486t^{79}+\\
&241704929497023593576284109748137t^{78}+401127329803571069200022148395060t^{77}+\\
&643475091559895257811475523869150t^{76}+998042999154123255509578916762251t^{75}+\\
&1497064498731184884738423828738826t^{74}+2172211233453091791403201171682487t^{73}+\\
&3049450385424532709259880563769891t^{72}+4142649580199365187088253032770042t^{71}+\\
&5446817040632498674709258423750752t^{70}+6932312597168634673342968879821758t^{69}+\\
&8541599450082782011722315254853863t^{68}+10189978291326827658936469293236257t^{67}+\\
&11771181819291335403215209136236758t^{66}+13167762713105561632909721570633733t^{65}+\\
&14265076272531025106827702213046251t^{64}+14966637400688288631941104298816390t^{63}+\\
&15208034778118744904852502416921288t^{62}+14966637400688288631941104298816390t^{61}+\\
&14265076272531025106827702213046251t^{60}+13167762713105561632909721570633733t^{59}+\\
\end{align*}

\begin{align*}
Total&[d;125](t) continued...\\
&11771181819291335403215209136236758t^{58}+10189978291326827658936469293236257t^{57}+\\
&8541599450082782011722315254853863t^{56}+6932312597168634673342968879821758t^{55}+\\
&5446817040632498674709258423750752t^{54}+4142649580199365187088253032770042t^{53}+\\
&3049450385424532709259880563769891t^{52}+2172211233453091791403201171682487t^{51}+\\
&1497064498731184884738423828738826t^{50}+998042999154123255509578916762251t^{49}+\\
&643475091559895257811475523869150t^{48}+401127329803571069200022148395060t^{47}+\\
&241704929497023593576284109748137t^{46}+140739579200798547810848407179486t^{45}+\\
&79166013300449183486752791791953t^{44}+43003760311355111831092568853122t^{43}+\\
&22550752358393534437019574995528t^{42}+11411224084970222152064822132446t^{41}+\\
&5569764136711656142477377352019t^{40}+2621065476099602847252984385458t^{39}+\\
&1188622715905633892156485804100t^{38}+519168542579472256031665746576t^{37}+\\
&218286773584550853413218320189t^{36}+88295773584762135474231228583t^{35}+\\
&34337245282963060080748456842t^{34}+12829300435392788915059242212t^{33}+\\
&4601814286608285713826377107t^{32}+1583419969585645756697355513t^{31}+\\
&522191692097394743906419238t^{30}+164902639609703309488079986t^{29}+\\
&49814339048764832197753486t^{28}+14379396838818630509486185t^{27}+\\
&3961670557633787406854497t^{26}+1040438732307841539649001t^{25}+\\
&260109683076981986458211t^{24}+61808241523238111266288t^{23}+\\
&13937152500343088195264t^{22}+2976867524344040005968t^{21}+601098250109006348605t^{20}+\\
&114494904782463078927t^{19}+20522671612153800248t^{18}+3452412046870263651t^{17}+\\
&543435229633787791t^{16}+79770308932154652t^{15}+10877769404828584t^{14}+\\
&1371970915393992t^{13}+159246624819695t^{12}+16911146021617t^{11}+\\
&1631777381270t^{10}+141893725177t^9+11009026889t^8+752765426t^7+44660526t^6+\\
&2253202t^5+94261t^4+3183t^3+90t^2+3t+1
\end{align*}


